Automated Reasoning and Detection of Specious Configuration in Large Systems with Symbolic Execution

Misconfiguration is a major cause of system failures. Prior solutions focus on detecting invalid settings that are introduced by user mistakes. But another type of misconfiguration that continues to haunt production services is specious configuration--settings that are valid but lead to unexpectedly poor performance in production. Such misconfigurations are subtle, so even careful administrators may fail to foresee them. We propose a tool called Violet to detect such misconfiguration. We realize the crux of specious configuration is that it causes some slow code path to be executed, but the bad performance effect cannot always be triggered. Violet thus takes a novel approach that uses selective symbolic execution to systematically reason about the performance effect of configuration parameters, their combination effect, and the relationship with input. Violet outputs a performance impact model for the automatic detection of poor configuration settings. We applied Violet on four large systems. To evaluate the effectiveness of Violet, we collect 17 real-world specious configuration cases. Violet detects 15 of them. Violet also identifies 9 unknown specious configurations.

==> section/background.tex <==
\section{Background}
\label{sec:background}


==> section/incidents.tex <==
\begin{table*}[t]
\centering
\small
\caption{Real-world gray failure service outages}
\label{tab:outage}
\begin{tabular}{@{}lp{12cm}ll@{}}
\toprule
{\bf No.} & {\bf Failure Description} & {\bf Cause} \\
\midrule
1 & Office 365 mail 8-hour service disruption: virus engine stuck in identifying 
some suspicious message, causing a significant backlog of valid email messages~\cite{office365_november_2013} & Bug+bad input \\
% 2 & Some active network elements experiencing gray failure mode together with increasing load cause severe mail service degradation~\cite{office365_november_2013} & Hardware fault+load \\
2 & Azure storage outage: During an automatic failover, the new primary loads state from disk but incorrectly sets the goal state to be empty and reformats nodes~\cite{azure_december_2012} & Bug+flaky disk \\
3 & AWS EBS 3+hour service outage: collection agents severe memory leak causes EBS processes to become stuck (unable to process I/O requests)~\cite{aws_october_2012} & Bug+resource \\
4 & Google Compute Engine 1-hour incident: new network links appear to be ready but unable to carry traffic; buggy load balancing mechanism fails to detect the unhealthy backends~\cite{google_june_2017} & Bug+network condition \\
5 & Entire ZooKeeper cluster near-deadlock due to a transient network issue and the problematic use of blocking I/O in a synchronized code block~\cite{ZooKeeperGrayFailure} & Bug+network condition\\
6 & Corrupt packets that escape checksum validation cause one critical thread of ZooKeeper to hit uncaught exceptions in deserializing the message~\cite{pagerduty_2014} & Bug+corrupt message\\
7 & Postgres cluster fails to fail over upon primary failure due to replica subprocess 
  crash and bad resource colocation rule~\cite{gocardless_october_2017} & Misconfig+failure event\\
8 & Twilio billing system incident: full synchronization requests from all Redis slaves 
to the Redis master at the same time after temporary network partition overload the Redis master; 
subsequent recovery of the master failed due to non-existent file, putting the master into read-only mode~\cite{twilio_july_2013} & Bug+network condition+file system\\
% 8 &  Azure Blob storage front-ends entering an infinite loop due to a bug exposed by a configuration change, unable to service requests~\cite{azure_2014_nov} & \\
  9 & Alibaba Elastic Container Service outage due to I/O hang errors, taking down numerous websites~\cite{alibaba_march_2019} & Bug+I/O stack\\
\bottomrule
\end{tabular}
\end{table*}

